Quantifying Carbon Emissions due to Online Third-Party Tracking

In the past decade, global warming made several headlines and turned the attention of the whole world to it. Carbon footprint is the main factor that drives greenhouse emissions up and results in the temperature increase of the planet with dire consequences. While the attention of the public is turned to reducing carbon emissions by transportation, food consumption and household activities, we ignore the contribution of CO2eq emissions produced by online activities. In the current information era, we spend a big amount of our days browsing online. This activity consumes electricity which in turn produces CO2eq. While website browsing contributes to the production of greenhouse gas emissions, the impact of the Internet on the environment is further exacerbated by the web-tracking practice. Indeed, most webpages are heavily loaded by tracking content used mostly for advertising, data analytics and usability improvements. This extra content implies big data transmissions which results in higher electricity consumption and thus higher greenhouse gas emissions. In this work, we focus on the overhead caused by web tracking and analyse both its network and carbon footprint. By leveraging the browsing telemetry of 100k users and the results of a crawling experiment of 2.7M websites, we find that web tracking increases data transmissions upwards of 21%, which in turn implies the additional emission of around 11 Mt of greenhouse gases in the atmosphere every year. We find such contribution to be far from negligible, and comparable to many activities of modern life, such as meat production, transportation, and even cryptocurrency mining. Our study also highlights that there exist significant inequalities when considering the footprint of different countries, website categories, and tracking organizations, with a few actors contributing to a much greater extent than the remaining ones.

==> Makefile <==
DOCNAME=paper

all: report

.PHONY: clean

report:
	pdflatex $(DOCNAME).tex
	bibtex -terse $(DOCNAME).aux
	pdflatex $(DOCNAME).tex
	pdflatex $(DOCNAME).tex

clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi


==> titleinfo.tex <==
%-- Use ``fancy'' to include the above Appears in... stuff
\thispagestyle{empty}
%\thispagestyle{fancy}

\title{Some Like it Hot: Quantifying Web-tracking \COtwo Footprint}
\author{}
%\author{Author1$^*$, Author2$^\dag$$^*$, Author3$^*$, 
%Author3$^\ddag$\thanks{Grants}\\ 
%$^*$Affiliation1 \quad $^\dag$Affiliation2 \quad $^\ddag$Affiliation3\\
%\email{\{email1, email2, email3\}@cmu.edu \, email4@foo.com} \\
%}

% Use \inst{1} after each author if different institutions
%\institute{
%Carnegie Mellon University,\\
%\email{\{none\}@cmu.edu}\\
%}
%\date{}
%\setlength{\headrulewidth}{0pt}
%\cfoot{}
\maketitle

%-- Use ``fancy'' to include the above Appears in... stuff
\thispagestyle{empty}
%\thispagestyle{fancy}

